Monte Carlo Tree Search for Verifying Reachability in Markov Decision Processes

The maximum reachability probabilities in a Markov decision process can be computed using value iteration (VI). Recently, simulation-based heuristic extensions of VI have been introduced, such as bounded real-time dynamic programming (BRTDP), which often manage to avoid explicit analysis of the whole state space while preserving guarantees on the computed result. In this paper, we introduce a new class of such heuristics, based on Monte Carlo tree search (MCTS), a technique celebrated in various machine-learning settings. We provide a spectrum of algorithms ranging from MCTS to BRTDP. We evaluate these techniques and show that for larger examples, where VI is no more applicable, our techniques are more broadly applicable than BRTDP with only a minor additional overhead.

==> macros.tex <==
\usepackage{xparse}
\usepackage{mathtools}
\usepackage{environ}

% == LATEX
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% == SPACE

%\usepackage{microtype}
%\renewcommand{\baselinestretch}{0.975} % >=0.97

%\newcommand{\spacefu}{\vspace*{-1.2em}}
%\newcommand{\spacefl}{\vspace*{-0.8em}}
%\newcommand{\myspace}{\vspace*{-0.5em}}

% == TODO

\NewDocumentCommand{\todo}{m}{%
	% Add to todo list
	\begin{tikzpicture}[remember picture, baseline=-0.75ex]%
	\node [coordinate] (inText) {};%
	\end{tikzpicture}%
	%
	% Make the margin par
	\marginpar{%
		\begin{tikzpicture}[remember picture, font=\scriptsize]%
		\draw node[draw=red, text width = 3.5cm, inner sep=0.3mm] (inNote){#1};%
		\end{tikzpicture}%
	}%
	\begin{tikzpicture}[remember picture, overlay]%
	\draw[draw=red]%
	([yshift=-0.2cm] inText)%
	% -| ([xshift=-0.05cm] inNote.west)%
	-| (inNote.south);%
	\end{tikzpicture}%
}%

% == SYMBOLS

\RequirePackage{marvosym}
\providecommand{\contradiction}{\Lightning}


% == BOOLEAN

\newcommand{\boolor}{\vee}
\newcommand{\booland}{\wedge}
\newcommand{\boolOr}{\bigvee}
\newcommand{\boolAnd}{\bigwedge}
\newcommand{\boolnot}{\lnot}


% == BASIC OPERATORS

\DeclarePairedDelimiter{\delimabs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\delimnorm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\delimpospart}{\lgroup}{\rgroup^+}
\DeclarePairedDelimiter{\delimnegpart}{\lgroup}{\rgroup^-}
\DeclarePairedDelimiterX{\deliminner}[2]{\lange}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\delimcardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\delimset}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\delimtuple}{(}{)}
\DeclarePairedDelimiter{\delimlistt}{[}{]}
\DeclarePairedDelimiter{\delimfun}{(}{)}

\NewDocumentCommand{\abs}{sm}{\IfBooleanTF{#1}{\delimabs{#2}}{\delimabs*{#2}}}
\NewDocumentCommand{\norm}{sm}{\IfBooleanTF{#1}{\delimnorm{#2}}{\delimnorm*{#2}}}
\NewDocumentCommand{\pospart}{sm}{\IfBooleanTF{#1}{\delimpospart{#2}}{\delimpospart*{#2}}}
\NewDocumentCommand{\negpart}{sm}{\IfBooleanTF{#1}{\delimnetpart{#2}}{\delimnetpart*{#2}}}
\NewDocumentCommand{\inner}{sm}{\IfBooleanTF{#1}{\deliminner{#2}}{\deliminner*{#2}}}
\NewDocumentCommand{\cardinality}{sm}{\IfBooleanTF{#1}{\delimcardinality{#2}}{\delimcardinality*{#2}}}
\NewDocumentCommand{\set}{sm}{\IfBooleanTF{#1}{\delimset{#2}}{\delimset*{#2}}}
\NewDocumentCommand{\tuple}{sm}{\IfBooleanTF{#1}{\delimtuple{#2}}{\delimtuple*{#2}}}
\NewDocumentCommand{\closure}{sm}{\IfBooleanTF{#1}{\delimclosure{#2}}{\delimclosure*{#2}}}
\NewDocumentCommand{\listt}{sm}{\IfBooleanTF{#1}{\delimlistt{#2}}{\delimlistt*{#2}}}
\NewDocumentCommand{\fun}{smm}{\IfBooleanTF{#1}{{#2}\delimfun{#3}}{{#2}\delimfun*{#3}}}
\NewDocumentCommand{\funMacro}{smm}{\IfNoValueTF{#3}{#1}{\fun{#2}{#3}}}

\DeclareMathOperator{\ExistsOp}{\exists}
\DeclareMathOperator{\ForallOp}{\forall}

\NewDocumentCommand{\Exists}{gg}{\IfNoValueTF{#1}{\ExistsOp}{\ExistsOp #1. \, #2}}
\NewDocumentCommand{\Forall}{gg}{\IfNoValueTF{#1}{\ForallOp}{\ForallOp #1. \, #2}}


% == SETS OPERATORS

\newcommand{\setcomplement}[1]{{#1}^c}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}


% == BASIC SETS

\newcommand{\Continuous}{C}
\newcommand{\Sobolev}{\mathcal{W}}
\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Domain}{\mathfrak{D}}
\newcommand{\Measures}{\mathcal{M}}
\newcommand{\Lebesgue}{\mathcal{L}}
\newcommand{\Hilb}{H}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Orlicz}{{\tilde{\Lebesgue}}}
\newcommand{\Distributions}{\mathcal{D}}


% == LIMITS

\NewDocumentCommand{\convto}{G{}}{\xrightarrow{#1}}
\NewDocumentCommand{\weakto}{G{}}{\xrightharpoonup{#1}}
\NewDocumentCommand{\weakstarto}{G{}}{\xrightharpoonup[*]{#1}}

% == OPERATORS

\newcommand{\gradient}{\nabla}
\newcommand{\laplacian}{\Delta}
\newcommand{\diff}{\partial}
\newcommand{\boundary}{\partial}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\distance}{dist}
\DeclareMathOperator{\esssup}{ess sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\capacity}{cap}
\DeclareMathOperator{\signum}{signum}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator{\opt}{opt}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum % TODO del

% == LOGIC

\newcommand{\ltl}{\operatorname{LTL}}
\newcommand{\ctl}{\operatorname{CTL}}
\newcommand{\pctl}{\operatorname{pCTL}}
\newcommand{\Next}{\varbigcirc}
\newcommand{\until}{\, \mathcal{U}}
\newcommand{\wrel}{\mathcal{W}}
\newcommand{\lang}[1]{\mathcal{L}(#1)}
\newcommand{\reach}{\Diamond}
\newcommand{\alws}{\Box}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\turn}{\mathsf{turn}}
\newcommand{\PQ}{\mathrm{PQ}}

% == COMPLEXITY
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}

% == PROBABILITY
\NewDocumentCommand{\distributions}{d()}{\funMacro{\mathcal{D}}{#1}}
\newcommand{\probability}{\mathbb{P}}
\newcommand{\expectation}{\mathbb{E}}

% == MC, MPD, Games

\newcommand{\gain}{g} %value
\newcommand{\bias}{b}
\newcommand{\stat}{q}
\newcommand{\outcomes}{\mathcal{O}}
\newcommand{\salgebra}{\mathcal{F}}
\newcommand{\mevent}{\mathcal{E}}
\newcommand{\pmin}{p_{\min}}
\newcommand{\rmax}{r_{\max}}
\newcommand{\MECs}{\mathsf{MEC}}
\newcommand{\GCs}{\mathsf{GC}}

\newcommand{\Ts}{\mathcal{T}}
\newcommand{\Mc}{\mathsf{M}}
\newcommand{\Mdp}{\mathcal{M}}
\newcommand{\Ctmdp}{\mathcal{C}}
\newcommand{\Pm}{\mathbf{P}}

\newcommand{\ap}{Ap}
\newcommand{\states}{S}
\newcommand{\inv}{\nu}
\newcommand{\lab}{L}

\newcommand{\edges}{E}
\newcommand{\statesone}{S^N}
\newcommand{\statestwo}{S_2}
\newcommand{\statesp}{S^P}
\newcommand{\initstate}{s_\textrm{init}}
\newcommand{\initdist}{\mu}
\newcommand{\trans}{\Delta}
\newcommand{\av}{\mathsf{Av}}
\newcommand{\rew}{r}
\newcommand{\lu}{\hat{l},\hat{u}}

\newcommand{\exit}[1]{\lambda(#1)}
\newcommand{\exitmax}[1]{\overline{\lambda}}
\newcommand{\ptime}[1]{\tau(#1)}

% = paths and strategies
\renewcommand{\path}{\rho}
\newcommand{\fpath}{w}
\newcommand{\Paths}{\Omega}
\newcommand{\straa}{\pi}
\newcommand{\straas}{\Pi}
\newcommand{\plays}{\mathsf{Plays}}
\newcommand{\play}{\mathsf{Play}}
\newcommand{\last}[1]{#1\mathord\downarrow}
\newcommand{\first}[1]{#1\mathord\uparrow}

\newcommand{\GM}{\ensuremath{\mathit{Tim}}\xspace} %generalised measurable schedulers
\newcommand{\late}{\ell}	%late schedulers
\newcommand{\early}{e}		%early schedulers
\newcommand{\x}{\nabla}		%\x \in {\late, \early}


% = probability

\newcommand{\inits}{\hat s}
\NewDocumentCommand{\actions}{d()}{{\IfNoValueTF{#1}{\mathit{Act}}{\fun{\mathit{Act}}{#1}}}}
\newcommand{\pat}{\omega}
\newcommand{\Pat}{\mathsf{Runs}}
\newcommand{\fpat}{w}
\newcommand{\mem}{\mathsf{M}}
\newcommand{\Cone}{\mathsf{Cone}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\mec}{\mathsf{MEC}}
\newcommand{\scc}{\mathsf{SCC}}
\newcommand{\bscc}{\mathsf{BSCC}}

\newcommand{\attractor}{\mathsf{prob1}}
\newcommand{\pr}{\mathbb P}
\renewcommand{\Pr}[3]{\pr^{#1}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\PrS}[3]{\pr^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\expected}{\mathbb{E}}
\newcommand{\expsucc}{\expected_\trans}
\newcommand{\Ex}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}
\newcommand{\ExS}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}


% == LOCAL

\newcommand{\push}{\mathrm{push}}
\newcommand{\pop}{\mathrm{pop}}
\newcommand{\topx}{\mathrm{top}}


\newcommand{\reward}{\vec{r}}
\newcommand{\ex}{\vecl{exp}}
\newcommand{\sat}{\vecl{sat}}
\newcommand{\satscalar}{\mathit{sat}}
\newcommand{\psat}{\vecl{pr}}%{\vec{p^{sat}}}
\newcommand{\psatscalar}{\mathit{pr}}%{\mathit{p^{sat}}}

\newcommand{\lrLim}[1]{\mathrm{lr}(#1)}  %\lr{rew}{run}
\newcommand{\lrSf}[1]{\mathrm{lr}_{\mathrm{sup}}(#1)}  %\lrS{rew}{run}
\newcommand{\lrIf}[1]{\mathrm{lr}_{\mathrm{inf}}(#1)}  %\lrI{rew}{run}
\newcommand{\lrInf}{\mathrm{lr}^{\mathrm{inf}}}  %\lrI{rew}{run}

\newcommand{\appear}{\textsf{Appear}}

\NewDocumentCommand{\spannorm}{m}{\fun{\operatorname{sp}}{#1}}


% == PROBLEM
%%\newcommand{\prr}[2]{\ifblank{#1}{\pr_{#2}}{\pr^{#1}_{#2}}}
%\newcommand{\reach}[2]{\Diamond^{\leq #1}#2}


\newcommand{\GetImportantPaths}[2]{\mathtt{GetImpPaths}(#1,#2)}
\newcommand{\SampleDiscretePath}[3]{\mathtt{SampleDiscretePath}(#1, #2, #3)}
\newcommand{\BackPropagate}{\mathtt{BackPropagate}}
\newcommand{\CBRTDP}{\mathtt{CTMDP-BRTDP}}
\newcommand{\Upper}[2]{U(#1,#2)}
\newcommand{\Lower}[2]{L(#1,#2)}
\newcommand{\variance}{\sigma}
\newcommand{\disstep}{\delta}
\newcommand{\transdiscret}[1]{\Delta_{#1}}

\newcommand{\nReach}{S_{0}}

